An Uplink Control Channel Design with Complementary Sequences for Unlicensed Bands

In this paper, two modulation schemes based on complementary sequences (CSs) are proposed for uplink control channels in unlicensed bands. These schemes address high peak-to-average-power ratio (PAPR) under non-contiguous resource allocation in the frequency domain and reduce the maximum PAPR to 3 dB. The first scheme allows the users to transmit a small amount of uplink control information (UCI) such as acknowledgment signals and does not introduce a trade-off between PAPR and co-channel interference (CCI). The second scheme, which enables up to 21 UCI bits for a single user or 11 UCI bits for three users in an interlace, is based on a new theorem introduced in this paper. This theorem leads distinct CSs compatible with a wide variety of resource allocations while capturing the inherent relationship between CSs and Reed-Muller (RM) codes, which makes CSs more useful for practical systems. The numerical results show that the proposed schemes maintain the low-PAPR benefits without increasing the error rate for non-contiguous resource allocations in the frequency domain.

==> v22_FINAL VERSION_arxiv/variables.tex <==
%% Originals
% Number Sets
\def\realsNonnegative{\mathbb{R}_{0}^{+}}
\def\realsNonnegative{\mathbb{R}_{0}^{+}}
\def\complexNumbers{\mathbb{C}}
\def\realNumbers{\mathbb{R}}
\def\integers{\mathbb{Z}}
\def\integersPositive{\mathbb{Z}^{+}}
\def\integersNonnegative{\mathbb{Z}_{0}^{+}}

% Constants
\def\constante{{\rm e}}
\def\constantj{{\rm j}}
\def\exponentialBase{\xi}
\def\lengthPillar{L}

\def\dminSeq{d_{\rm min}^{\rm e}}
\def\peakCrossCorrelatation[#1]{\rho_{\text{peak}}#1}


\def\constante{{\rm e}}
\def\constantj{{\rm j}}
\def\exponentialBase{\xi}
\def\constanti{{\rm i}}
\def\constantMinusi{{\rm j}}
\def\constantOne{{\rm +}}
\def\constantMinusOne{{\rm -}}

% Scalars, variables, indices
\def\upsampleVarA{k}
\def\upsampleVarB{l}
\def\paddingVar{d}
\def\lagForCorrelation{\tau}
\def\unitSequences{G_0}
\def\dunitSequences{A_0}

\def\unmodVar{z}
\def\indexEleOfSeq{\iota}
\def\indexIteration{n}
\def\indexIterationdot{\bar{n}}
\def\indexIterationANF{l}
\def\indexChoosen{\ell}
\def\indexChoosenOne{\ell_1}
\def\indexChoosenTwo{\ell_2}
\def\indexFirstOrderMonomial{j}
\def\indexMonomial{k}
\def\orderMonomial[#1]{k_{#1}}
\def\coeffientsANF[#1]{c_{#1}}
\def\polyVariable{z}
\def\polyVariableIt{w}
\def\numberOfIterations{m}
\def\numberOfPointsForPSK{H}
\def\modulationSymbolF[#1]{m_{#1}}
\def\cardinalitySetOfOperators[#1]{{H}_{#1}}

\def\numberSequencesDifferentThanLEngthOne{A}
\def\numberSequencesNotColinear{B}

\def\varMonomial{x}
\def\monomial[#1]{x_{#1}}
\def\varUpsample{U}

\def\lengthData{M}
\def\lengthGaGb{N}
\def\lengthGcGd{M}
\def\lengthGcGdIterative[#1]{M_{#1}}
\def\lengthGcGdContIterative[#1]{\dot{M}_{#1}}

\def\scaleAexp[#1]{a_{#1}}
\def\scaleBexp[#1]{b_{#1}}
\def\scaleEexp[#1]{e_{#1}}
\def\angleexp[#1]{c_{#1}}
\def\angleexpAll[#1]{k_{#1}}
\def\angleScaleAexp[#1]{\dot{c}_{#1}}
\def\angleScaleBexp[#1]{\ddot{c}_{#1}}
\def\arbitraryScaleE{e'}
\def\arbitraryPhaseA{c'}
\def\arbitraryPhaseB{c''}
\def\arbitraryPhaseK{k'}
\def\separationGolay[#1]{d_{#1}}


\def\eleGa[#1]{{a}_{#1}}
\def\eleGb[#1]{{b}_{#1}}
\def\elex[#1]{{x}_{#1}}
\def\eles[#1]{{s}_{#1}}
\def\eley[#1]{{y}_{#1}}

\def\apac[#1][#2]{\rho_{#1}(#2)}
\def\apacPositive[#1][#2]{\rho^{+}_{#1}(#2)}
\def\binaryAsignment[#1][#2]{b_{#1}^{(#2)}}

\def\eleSeqf[#1]{{f}_{#1}}
\def\eleSeqg[#1]{{g}_{#1}}
\def\eleSeqcf[#1]{{c}_{f,#1}}
\def\eleSeqcg[#1]{{c}_{g,#1}}

\def\scaleA[#1]{\alpha_{#1}}
\def\scaleB[#1]{\beta_{#1}}
\def\angleGolay[#1]{\omega_{#1}}
\def\angleScaleA[#1][#2]{\dot{\omega}_{#1}^{#2}}
\def\angleScaleB[#1][#2]{\ddot{\omega}_{#1}^{#2}}
\def\permutationShift[#1]{{\psi_{#1}}}
\def\permutationMono[#1]{{\pi_{#1}}}
\def\permutationUpsample[#1]{{\kappa_{#1}}}
\def\permutationOrderEle[#1]{{\phi_{#1}}}

\def\symbolDuration{T_{\rm s}}
\def\timeVar{t}
\def\PAPR{PAPR}
\def\cubicMetric{CM}

\def\vNorm{v_{\rm norm}(\timeVar)}
\def\vNormCubic{v^3_{\rm norm}(\timeVar)}


\def\thershold{\beta}
\def\upsampleValueU{u}
\def\seedA{\mathcal{S}_{\rm c}''}
\def\seedB{\mathcal{S}_{\rm d}''}
\def\seedAp{\mathcal{S}_{\rm c}'}
\def\seedBp{{\mathcal{S}_{\rm d}'}}
\def\seedSize{V}
\def\seedSizeEq{W}
\def\setS{\mathbb{S}}
\def\indexForFirst{\dot{u}}
\def\indexForSecond{\dot{v}}
\def\correlationCalc{\alpha}

\def\setC{\mathcal{C}}
\def\setD{\mathcal{D}}
\def\setQ{\mathcal{Q}_1}
\def\setQr{\mathcal{Q}_2}
\def\numberOfSequences{K}
\def\indexSequence{i}

\def\funczArbitrary[#1]{z(#1)}
\def\funcaArbitrary[#1]{a(#1)}
\def\funcbArbitrary[#1]{b(#1)}
\def\coefficientArbitrary[#1]{k_{#1}}

\def\indexRB{k}

\def\sqrtofNumPointsInQuad{s}
\def\setOfQAM{\mathbb{S}_{\rm QAM}}
\def\inphaseIndex{u}
\def\quadIndex{v}
\def\anotherForIndex{w}
\def\anotherTwoForIndex{t}
\def\Nquad{N_{\rm quad}}
\def\Squad{S_{\rm quad}}
\def\Nh{N_{\rm h}}
\def\Sh{S_{\rm h}}
\def\Nnh{N_{\rm nh}}
\def\Snhplus{S_{\rm nh}^{+}}
\def\Ntri{N_{\rm tri}}
\def\Stri{S_{\rm tri}}
\def\Snhnegative{S_{\rm nh}^{-}}
\def\pointQAM{p}
\def\sympointQAM{p'}
\def\anotherPointQAM{p''}
\def\distanceToPoint[#1]{d_{#1}}
\def\ratioBetweenDistanceAndInner[#1]{l_{#1}}
\def\angleBetweenPointAndXaxis[#1]{\theta_{#1}}
\def\angleBetweenPointAndXYDiagonal[#1]{\psi_{#1}}
\def\angleBetweenPointAndSymPoint[#1]{\xi_{#1}}


\def\numberOfClusters{N_{\rm rb}}
\def\RBsize{N_{\rm sc}}
\def\numberOfNulls{N_{\rm null}}

\def\correlationMetric{\rho}
\def\dftSize{N_{\rm IDFT}}


% Sequences, vectors
\def\vecArrangement[#1]{\textbf{b}_{#1}}

\def\encodedVector{\textit{\textbf{g}}}
\def\seqGa{\textit{\textbf{a}}}
\def\seqGb{\textit{\textbf{b}}}
\def\seqGaIt[#1]{\textit{\textbf{a}}^{(#1)}}
\def\seqGbIt[#1]{\textit{\textbf{b}}^{(#1)}}
\def\seqGc{\textit{\textbf{c}}}
\def\seqGd{\textit{\textbf{d}}}
\def\seedSeqGcCandidate[#1]{{\seqGc_{#1}''}}
\def\seedSeqGdCandidate[#1]{{\seqGd_{#1}''}}
\def\seqGcCandidate[#1]{{\seqGc_{#1}'}}
\def\seqGdCandidate[#1]{{\seqGd_{#1}'}}
\def\seqGcRecursion[#1]{{\seqGc_{#1}}}
\def\seqGdRecursion[#1]{{\seqGd_{#1}}}
\def\seqGcContRecursion[#1]{{\dot{\seqGc}_{#1}}}
\def\seqGdContRecursion[#1]{{\dot{\seqGd}_{#1}}}


\def\seqGcTildeRecursion[#1]{{\tilde{\seqGc}_{#1}}}
\def\seqGdTildeRecursion[#1]{{\tilde{\seqGd}_{#1}}}

\def\seqPermutationShift{\bm{\psi}}
\def\seqPermutationCompShift{\bm{\pi}}
\def\seqPermutationOrder{\bm{\phi}}
\def\seqPermutationUpsample{\bm{\kappa}}

\def\seqGf{\textit{\textbf{t}}}
\def\seqGg{\textit{\textbf{r}}}
\def\seqGx{\textit{\textbf{x}}}
\def\seqGy{\textit{\textbf{y}}}
\def\seqGs{\textit{\textbf{s}}}
\def\seqGsShift[#1]{{\textit{\textbf{s}}}_{#1}}
%
%\def\seqGf[#1]{\textit{\textbf{f}}_{#1}}
%\def\seqGg[#1]{\textit{\textbf{g}}_{#1}}
%\def\seqGfdot[#1]{\bar{\textit{\textbf{f}}}_{#1}}
%\def\seqGgdot[#1]{\bar{\textit{\textbf{g}}}_{#1}}


\def\seqf{\textit{\textbf{f}}}
\def\seqData{\textit{\textbf{s}}}

\def\seqSub[#1]{\textit{\textbf{h}}_{#1}}

\def\seqFirstOrderMonomial[#1]{\textit{\textbf{m}}_{#1}}
\def\seqx{\textit{\textbf{x}}}
\def\seqk{\textit{\textbf{k}}}
\def\seqToBeModulated[#1]{\textit{\textbf{s}}_{#1}}
\def\seqCelep[#1][#2]{\phi_{#1#2}}
\def\seqDelep[#1][#2]{\theta_{#1#2}}





% Operators
\def\flipConjugate[#1]{{{\tilde{#1}}}}
\def\expectationOperator[#1]{{\mathbb{E}}[#1]}
\def\operator[#1][#2]{\mathcal{O}_{#1}^{(#2)}}
\def\operatordot[#1][#2]{\bar{\mathcal{O}}_{#1}^{(#2)}}

\def\compositeOperatorF[#1][#2]{{F}_{#1}{(#2)}}
\def\compositeOperatorG[#1][#2]{{G}_{#1}{(#2)}}
\def\compositeOperatorFdot[#1][#2]{\bar{F}_{#1}{(#2)}}
\def\compositeOperatorGdot[#1][#2]{\bar{G}_{#1}{(#2)}}


\def\compositeOperatorFcd[#1][#2]{{F}_{{\rm cd\tilde{c}\tilde{d}},#1}{(#2)}}
\def\compositeOperatorGcd[#1][#2]{{G}_{{\rm cd\tilde{c}\tilde{d}},#1}{(#2)}}

\def\compositeOperatorFangle[#1][#2]{{F}_{{\rm comp},#1}{(#2)}}
\def\compositeOperatorGangle[#1][#2]{{G}_{{\rm comp},#1}{(#2)}}

\def\setOfOperators[#1]{{\mathfrak{J}}_{#1}}

\def\operatorBinary[#1][#2]{O_{#1}^{(#2)}}
\def\operatorSign[#1][#2]{{\rm S}_{#1}^{(#2)}}
\def\operatorScaleA[#1][#2]{{\rm{A}}_{#1}^{(#2)}}
\def\operatorScaleB[#1][#2]{{\rm{B}}_{#1}^{(#2)}}
\def\operatorAngle[#1][#2]{\Omega_{#1}^{(#2)}}
\def\operatorSeparation[#1][#2]{\Delta_{#1}^{(#2)}}
\def\operatorOrderA[#1][#2]{\dot{\rm O}_{#1}^{(#2)}}
\def\operatorOrderB[#1][#2]{\ddot{\rm O}_{#1}^{(#2)}}
\def\operatorAngleScaleA[#1][#2]{\dot{\Omega}_{#1}^{(#2)}}
%\def\operatorAngleScaleB[#1][#2]{\ddot{\Omega}_{#1}^{(#2)}}
\def\operatorAngleScaleB[#1][#2]{{\Omega}_{#1}^{(#2)}}
\def\operatorAngleConjScaleA[#1][#2]{\dot{\Upsilon}_{#1}^{(#2)}}
\def\operatorAngleConjScaleB[#1][#2]{\ddot{\Upsilon}_{#1}^{(#2)}}

\def\operatorOrderC[#1][#2]{{\rm C}_{#1}^{(#2)}}
\def\operatorOrderD[#1][#2]{{\rm D}_{#1}^{(#2)}}
\def\operatorOrderCtilde[#1][#2]{{\rm \tilde{C}}_{#1}^{(#2)}}
\def\operatorOrderDtilde[#1][#2]{{\rm \tilde{D}}_{#1}^{(#2)}}

\def\upsampleOp[#1][#2]{{\uparrow_{#1}\{#2\}}}
\def\shift[#1]{r_{#1}}
\def\operatorRMS[#1]{{\rm rms}\{#1\}}
\def\operationIDFT[#1][#2]{{\rm IDFT}\{#1,#2\}}
\def\operationMAX[#1]{{\rm max}\{#1\}}

% Functions
\def\functionSpace{\mathcal{F}}
\def\functionf[#1]{p^{(#1)}}
\def\functiong[#1]{q^{(#1)}}
\def\functionh{r}
\def\functionfdot[#1]{\bar{p}_{\indexIterationANF}^{(#1)}}
\def\functiongdot[#1]{\bar{q}_{\indexIterationANF}^{(#1)}}

\def\funcfForCommonAmplitude{c_{\rm r}}
\def\funcfForPartAAmplitude{f_{\rm r}}
\def\funcfForPartBAmplitude{g_{\rm r}}
\def\funcfForCommonPhase{c_{\rm i}}
\def\funcfForCommonPhaseA{f_{\rm i}}
\def\funcfForCommonPhaseB{g_{\rm i}}
\def\funcfForCommonShift{f_{\rm s}}
\def\funcForCommonOrder{p_{\rm o}}
\def\funcfForCommonOrder{f_{\rm o}}
\def\funcgForCommonOrder{g_{\rm o}}
\def\funcfForTuryn{f_{\rm f}}
\def\funcfForTurynPart[#1]{f_{{\rm f},#1}}
\def\funcgForTurynPart[#1]{g_{{\rm f},#1}}
\def\funcfForTurynC{f_{\rm c}}
\def\funcfForTurynCtilde{f_{\rm \tilde{c}}}
\def\funcfForTurynD{f_{\rm d}}
\def\funcfForTurynDtilde{f_{\rm \tilde{d}}}


\def\funcfForFinalPhase{f_{\rm i}}
\def\funcgForFinalPhase{g_{\rm i}}
\def\funcfForFinalAmplitude{f_{\rm r}}

\def\funcfForANF{f}
\def\funcGfForANF[#1]{f_{#1}}
\def\funcGgForANF[#1]{g_{#1}}

\def\funcGfForC[#1]{f_{{\rm c}, #1}}
\def\funcGgForC[#1]{g_{{\rm c}, #1}}
\def\funcGfForD[#1]{f_{{\rm d}, #1}}
\def\funcGgForD[#1]{g_{{\rm d}, #1}}
\def\funcGfForCtilde[#1]{f_{{\rm \tilde{c}}, #1}}
\def\funcGgForCtilde[#1]{g_{{\rm \tilde{c}}, #1}}
\def\funcGfForDtilde[#1]{f_{{\rm \tilde{d}}, #1}}
\def\funcGgForDtilde[#1]{g_{{\rm \tilde{d}}, #1}}



\def\polySeq[#1][#2]{p_{#1}(#2)}



\def\funcfForANFsign{f_{\rm sign}}
\def\funcgForANFsign{g_{\rm sign}}
\def\funcfForANFsequenceA{f_{\rm order,a}}
\def\funcgForANFsequenceA{g_{\rm order,a}}
\def\funcfForANFsequenceB{f_{\rm order,b}}
\def\funcgForANFsequenceB{g_{\rm order,b}}
\def\funcfForANFphase{f_{\rm phase}}
\def\funcgForANFphase{g_{\rm phase}}
\def\funcfForANFamplitudeA{f_{\rm scale,a}}
\def\funcgForANFamplitudeA{g_{\rm scale,a}}

\def\funcfForANFphaseA{f_{\rm phase,a}}
\def\funcgForANFphaseA{g_{\rm phase,a}}
\def\funcfForANFphaseAconj{f_{\rm phase,a^*}}
\def\funcgForANFphaseAconj{g_{\rm phase,a^*}}
\def\funcfForANFphaseB{f_{\rm phase,b}}
\def\funcgForANFphaseB{g_{\rm phase,b}}
\def\funcfForANFphaseBconj{f_{\rm phase,b^*}}
\def\funcgForANFphaseBconj{g_{\rm phase,b^*}}


\def\funcfForANFamplitudeB{f_{\rm scale,b}}
\def\funcgForANFamplitudeB{g_{\rm scale,b}}
\def\funcfForANFseparation{f_{\rm shift}}
\def\funcgForANFseparation{g_{\rm shift}}


